Opinion dynamics and consensus formation in a Deffuant model with extremists and moderates

Among the different disciplines in the social, behavioral and economic sciences, a fundamental class of problems is related to the prediction of the final state of the presence of individual opinions in a large population. The main aspects investigated in the opinion dynamics are related to the possibility of reaching an agreement and the time needed. In general a consensus model allows to understand if a set of interacting agents can reach a consensus when choosing among several options: political vote, opinions, cultural features are well-known examples of them. Opinion dynamics models then can be seen as a sub-set of consensus models, when the options to choose from are opinions and the possible social consensus to be reached is the opinion agreement. Moreover, in large populations it is intuitive to find moderates, whose opinion is not at the extremes of the political opinion spectrum. Due to the wide range of their empirical presence, the study of their influence in the opinion dynamics processes is very important to enhance the comprehension of the political opinions evolution in large populations. The Deffuant model is aimed at studying consensus formation assuming that the opinion distribution of a population evolves via a sequence of random pairwise encounters. In this work we strive to extend the classical Deffuant model with the presence of moderates in addition to the extremists, so as to study the emergence of consensus with different initial configurations of opinions and parameters. Therefore, we assess the role and the importance of the moderates for the appearance of consensus in the opinion dynamics processes within in large populations. We show that the population behavior is affected by the presence of a critical number of moderates, in specific configurations of the model parameters: when this threshold is reached the opinions in the population progressively converge

==> bib.tex <==
@Article{doi:10.1080/01621459.1974.10480137,
  author    = {Morris H. Degroot},
  title     = {Reaching a Consensus},
  journal   = {Journal of the American Statistical Association},
  year      = {1974},
  volume    = {69},
  number    = {345},
  pages     = {118-121},
  doi       = {10.1080/01621459.1974.10480137},
  eprint    = {https://amstat.tandfonline.com/doi/pdf/10.1080/016214\\59.1974.10480137},
  publisher = {Taylor \& Francis},
  url       = { 
        https://amstat.tandfonline.com/doi/abs/10.1080/01621459.1974.10480137
    
},
}

@article{doi:10.1086/228313,
author = {Oliver, Pamela and Marwell, Gerald and Teixeira, Ruy},
title = {A Theory of the Critical Mass. I. Interdependence, Group Heterogeneity, and the Production of Collective Action},
journal = {American Journal of Sociology},
volume = {91},
number = {3},
pages = {522-556},
year = {1985},
doi = {10.1086/228313},

URL = { 
        https://doi.org/10.1086/228313
    
},
eprint = { 
        https://doi.org/10.1086/228313
    
}
,
    abstract = { Collective action usually depends on a "critical mass" that behaves differently from typical group members. Sometimes the critical mass provides some level of the good for others who do nothing, while at other times the critical mass pays the start-up costs and induces widespread collective action. Formal analysis supplemented by simulations shows that the first scenario is most likely when the production function relating inputs of resource contributions to outputs of a collective good is decelerating (characterized by diminishing marginal returns), whereas the second scenario is most likely when the production function is accelerating (characterized by increasing marginal returns). Decelerating production functions yield either surpluses of contributors or order effects in which contributions are maximized if the least interested contribute first, thus generating strategic gaming and competition among potential contributors. The start-up costs in accelerating production functions create severe feasibility problems for collective action, and contractual or conventional resolutions to collective dilemmas are most appropriate when the production function is accelerating. }
}

@article{10.2307/2959329,
 ISSN = {00911798},
 URL = {http://www.jstor.org/stable/2959329},
 abstract = {A theorem exhibiting the duality between certain infinite systems of interacting stochastic processes and a type of branching process is proved. This duality is then used to study the ergodic properties of the infinite system. In the case of the vector model a complete understanding of the ergodic behavior is obtained.},
 author = {Richard A. Holley and Thomas M. Liggett},
 journal = {The Annals of Probability},
 number = {4},
 pages = {643--663},
 publisher = {Institute of Mathematical Statistics},
 title = {Ergodic Theorems for Weakly Interacting Infinite Systems and the Voter Model},
 volume = {3},
 year = {1975}
}

@article{GRANOVSKY199523,
title = "The noisy voter model",
journal = "Stochastic Processes and their Applications",
volume = "55",
number = "1",
pages = "23 - 43",
year = "1995",
issn = "0304-4149",
doi = "https://doi.org/10.1016/0304-4149(94)00035-R",
url = "http://www.sciencedirect.com/science/article/pii/030441499400035R",
author = "Boris L. Granovsky and Neal Madras",
keywords = "Voter model, Noisy voter model, Graph, Duality, Moran model, Transient behaviour, Random walk, Green function, Critical exponents, Scaling",
abstract = "The noisy voter model is a spin system on a graph which may be obtained from the basic voter model by adding spontaneous flipping from 0 to 1 and from 1 to 0 at each site. Using duality, we obtain exact formulas for some important time-dependent and equilibrium functionals of this process. By letting the spontaneous flip rates tend to zero, we get the basic voter model, and we calculate the exact critical exponents associated with this “phase transition”. Finally, we use the noisy voter model to present an alternate view of a result due to Cox and Griffeath on clustering in the two-dimensional basic voter model."
}

@article{Castellano_2003,
	doi = {10.1209/epl/i2003-00490-0},
	url = {https://doi.org/10.1209%2Fepl%2Fi2003-00490-0},
	year = 2003,
	month = {jul},
	publisher = {{IOP} Publishing},
	volume = {63},
	number = {1},
	pages = {153--158},
	author = {C Castellano and D Vilone and A Vespignani},
	title = {Incomplete ordering of the voter model on small-world networks},
	journal = {Europhysics Letters ({EPL})},
	abstract = {We investigate how the topology of small-world networks affects
the dynamics of the voter model for opinion formation. We show
that, contrary to what occurs on regular topologies with local
interactions, the voter model on small-world networks does not
display the emergence of complete order in the thermodynamic
limit. The system settles in a stationary state with coexisting
opinions whose lifetime diverges with the system size. Hence the
nontrivial connectivity pattern leads to the counterintuitive
conclusion that long-range connections inhibit the ordering
process. However, for networks of finite size, for which full
uniformity is reached, the ordering process takes a time shorter
than on a regular lattice of the same size.}
}

@article{PhysRevE.69.016109,
  title = {Solution of voter model dynamics on annealed small-world networks},
  author = {Vilone, Daniele and Castellano, Claudio},
  journal = {Phys. Rev. E},
  volume = {69},
  issue = {1},
  pages = {016109},
  numpages = {8},
  year = {2004},
  month = {Jan},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevE.69.016109},
  url = {https://link.aps.org/doi/10.1103/PhysRevE.69.016109}
}

@article{PhysRevLett.112.158701,
  title = {Is the Voter Model a Model for Voters?},
  author = {Fern\'andez-Gracia, Juan and Suchecki, Krzysztof and Ramasco, Jos\'e J. and San Miguel, Maxi and Egu\'{\i}luz, V\'{\i}ctor M.},
  journal = {Phys. Rev. Lett.},
  volume = {112},
  issue = {15},
  pages = {158701},
  numpages = {5},
  year = {2014},
  month = {Apr},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.112.158701},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.112.158701}
}

@article{STAUFFER200293,
title = "Sociophysics: the Sznajd model and its applications",
journal = "Computer Physics Communications",
volume = "146",
number = "1",
pages = "93 - 98",
year = "2002",
note = "Proceedings of the STATPHYS Satellite Conference: Challenges in Computational Statistical Physics in teh 21st Century",
issn = "0010-4655",
doi = "https://doi.org/10.1016/S0010-4655(02)00439-3",
url = "http://www.sciencedirect.com/science/article/pii/S0010465502004393",
author = "Dietrich Stauffer",
abstract = "The Sznajd model in one year has found several followers. An isolated person does not convince others; a group of people sharing the same opinions influences the neighbours much more easily. Thus on a square lattice, with variables +1 (Democrats) and −1 (Republicans) on every lattice site, a pair (or plaquette) of neighbours convinces its six (eight) nearest neighbours of its own opinion if and only if all members of the pair (plaquette) share the same opinion. The generalization to many possible states is used to explain the distribution of votes among candidates in Brazilian local elections."
}

@article{doi:10.1177/0022002797041002001,
author = {Robert Axelrod},
title ={The Dissemination of Culture: A Model with Local Convergence and Global Polarization},
journal = {Journal of Conflict Resolution},
volume = {41},
number = {2},
pages = {203-226},
year = {1997},
doi = {10.1177/0022002797041002001},

URL = { 
        https://doi.org/10.1177/0022002797041002001
    
},
eprint = { 
        https://doi.org/10.1177/0022002797041002001
    
}
,
    abstract = { Despite tendencies toward convergence, differences between individuals and groups continue to exist in beliefs, attitudes, and behavior. An agent-based adaptive model reveals the effects of a mechanism of convergent social influence. The actors are placed at fixed sites. The basic premise is that the more similar an actor is to a neighbor, the more likely that that actor will adopt one of the neighbor's traits. Unlike previous models of social influence or cultural change that treat features one at a time, the proposed model takes into account the interaction between different features. The model illustrates how local convergence can generate global polarization. Simulations show that the number of stable homogeneous regions decreases with the number of features, increases with the number of alternative traits per feature, decreases with the range of interaction, and (most surprisingly) decreases when the geographic territory grows beyond a certain size. }
}

@article{doi:10.1086/226707,
author = {Granovetter, Mark},
title = {Threshold Models of Collective Behavior},
journal = {American Journal of Sociology},
volume = {83},
number = {6},
pages = {1420-1443},
year = {1978},
doi = {10.1086/226707},

URL = { 
        https://doi.org/10.1086/226707
    
},
eprint = { 
        https://doi.org/10.1086/226707
    
}
,
    abstract = { Models of collective behavior are developed for situations where actors have two alternatives and the costs and/or benefits of each depend on how many other actors choose which alternative. The key concept is that of "threshold": the number or proportion of others who must make one decision before a given actor does so; this is the point where net benefits begin to exceed net costs for that particular actor. Beginning with a frequency distribution of thresholds, the models allow calculation of the ultimate or "equilibrium" number making each decision. The stability of equilibrium results against various possible changes in threshold distributions is considered. Stress is placed on the importance of exact distributions distributions for outcomes. Groups with similar average preferences may generate very different results; hence it is hazardous to infer individual dispositions from aggregate outcomes or to assume that behavior was directed by ultimately agreed-upon norms. Suggested applications are to riot behavior, innovation and rumor diffusion, strikes, voting, and migration. Issues of measurement, falsification, and verification are discussed. }
}

@article{doi:10.1142/S0219525900000078,
author = {Deffuant, Guillaume and Neau, David and Amblard, Frederic and Weisbuch, Gérard},
title = {Mixing beliefs among interacting agents},
journal = {Advances in Complex Systems},
volume = {03},
number = {01n04},
pages = {87-98},
year = {2000},
doi = {10.1142/S0219525900000078},

URL = { 
        https://doi.org/10.1142/S0219525900000078
    
},
eprint = { 
        https://doi.org/10.1142/S0219525900000078
    
}
,
    abstract = { We present a model of opinion dynamics in which agents adjust continuous opinions as a result of random binary encounters whenever their difference in opinion is below a given threshold. High thresholds yield convergence of opinions towards an average opinion, whereas low thresholds result in several opinion clusters: members of the same cluster share the same opinion but are no longer influenced by members of other clusters. }
}

@article{doi:10.1002/cplx.10031,
author = {Weisbuch, Gérard and Deffuant, Guillaume and Amblard, Frédéric and Nadal, Jean-Pierre},
title = {Meet, discuss, and segregate!},
journal = {Complexity},
volume = {7},
number = {3},
pages = {55-63},
keywords = {opinion dynamics, heterogeneous agents, bounded confidence},
doi = {10.1002/cplx.10031},
url = {https://onlinelibrary.wiley.com/doi/abs/10.1002/cplx.10031},
eprint = {https://onlinelibrary.wiley.com/doi/pdf/10.1002/cplx.10031},
abstract = {Abstract We present a model of opinion dynamics in which agents adjust continuous opinions as a result of random binary encounters whenever their difference in opinion is below a given threshold. High thresholds yield convergence of opinions toward an average opinion, whereas low thresholds result in several opinion clusters. The model is further generalized to network interactions, threshold heterogeneity, adaptive thresholds, and binary strings of opinions. © 2002 Wiley Periodicals, Inc.},
year = {2002}
}

@article{10.1093/biomet/60.3.581,
    author = {Clifford, Peter and Sudbury, Aidan},
    title = "{A model for spatial conflict}",
    journal = {Biometrika},
    volume = {60},
    number = {3},
    pages = {581-588},
    year = {1973},
    month = {12},
    abstract = "{SUMMARYTwo species compete for territory along their mutual boundary. The species are fairly matched and the result of conflict is the invasion by one of the species of territory held by the other. A simple stochastic model for this process is described and rules are given for the calculation, as a function of time, of the probabilities that individual territories and groups of territories are held by a single species. Asymptotic results are given for the pattern of territories held by a single species, and here a remarkable distinction is seen between the cases of one-dimensional and two-dimensional competition and the case of three-dimensional competition. The process of invasion is contrasted with two relatively benign processes, that in which an exchange of territories is arranged and that in which a spatial alternation of species may be beneficial to the community. The implications of the long-term behaviour of such processes are discussed. It is suggested further that, under certain ideal conditions, it may be possible to estimate the duration of a spatial struggle for life by observing at some time the configuration of territories held by each species.}",
    issn = {0006-3444},
    doi = {10.1093/biomet/60.3.581},
    url = {https://doi.org/10.1093/biomet/60.3.581},
    eprint = {https://academic.oup.com/biomet/article-pdf/60/3/581/576759/60-3-581.pdf},
}

@article{10.2307/2959329,
 ISSN = {00911798},
 URL = {http://www.jstor.org/stable/2959329},
 abstract = {A theorem exhibiting the duality between certain infinite systems of interacting stochastic processes and a type of branching process is proved. This duality is then used to study the ergodic properties of the infinite system. In the case of the vector model a complete understanding of the ergodic behavior is obtained.},
 author = {Richard A. Holley and Thomas M. Liggett},
 journal = {The Annals of Probability},
 number = {4},
 pages = {643--663},
 publisher = {Institute of Mathematical Statistics},
 title = {Ergodic Theorems for Weakly Interacting Infinite Systems and the Voter Model},
 volume = {3},
 year = {1975}
}

@article{doi:10.1142/S0129183106010108,
author = {Jacobeimer, Dirk},
title = {FOCUSING OF OPINIONS IN THE DEFFUANT MODEL: FIRST IMPRESSION COUNTS},
journal = {International Journal of Modern Physics C},
volume = {17},
number = {12},
pages = {1801-1808},
year = {2006},
doi = {10.1142/S0129183106010108},

URL = { 
        https://doi.org/10.1142/S0129183106010108
    
},
eprint = { 
        https://doi.org/10.1142/S0129183106010108
    
}
,
    abstract = { This paper treats the opinion dynamics of an unequal, initial opinion distribution. We simulate the Deffuant model on a directed Barabási–Albert network with discrete opinions and several subjects. We notice a focusing of the the resulting opinion distribution during the simulation towards the average value of the initial opinion distribution. A small change of the focusing is seen. A dependency of this change on the number of subjects and opinions is detected and indicates the change as a consequence of discretization of the opinions. Hereby the average value of the initial opinion distribution can be identified as the guide of opinion forming. }
}

@article{doi:10.1002/cplx.10031,
author = {Weisbuch, Gérard and Deffuant, Guillaume and Amblard, Frédéric and Nadal, Jean-Pierre},
title = {Meet, discuss, and segregate!},
journal = {Complexity},
volume = {7},
number = {3},
pages = {55-63},
keywords = {opinion dynamics, heterogeneous agents, bounded confidence},
doi = {10.1002/cplx.10031},
url = {https://onlinelibrary.wiley.com/doi/abs/10.1002/cplx.10031},
eprint = {https://onlinelibrary.wiley.com/doi/pdf/10.1002/cplx.10031},
abstract = {Abstract We present a model of opinion dynamics in which agents adjust continuous opinions as a result of random binary encounters whenever their difference in opinion is below a given threshold. High thresholds yield convergence of opinions toward an average opinion, whereas low thresholds result in several opinion clusters. The model is further generalized to network interactions, threshold heterogeneity, adaptive thresholds, and binary strings of opinions. © 2002 Wiley Periodicals, Inc.},
year = {2002}
}

@article{doi:10.1002/cplx.20018,
author = {Laguna, M. F. and Abramson, Guillermo and Zanette, Damián H.},
title = {Minorities in a model for opinion formation},
journal = {Complexity},
volume = {9},
number = {4},
pages = {31-36},
keywords = {collective state, synchronization effect, opinion formation},
doi = {10.1002/cplx.20018},
url = {https://onlinelibrary.wiley.com/doi/abs/10.1002/cplx.20018},
eprint = {https://onlinelibrary.wiley.com/doi/pdf/10.1002/cplx.20018},
abstract = {Abstract We study a model for social influence in which the agents' opinion is a continuous variable [G. Weisbuch et al., Complexity 2002, 7(2), 55]. The convergent opinion adjustment process takes place as a result of random binary encounters whenever the difference between agents' opinions is below a given threshold. The inhomogeneity in the dynamics gives rise to a complex steady state structure, which is also highly dependent on the threshold and on the convergence parameter of the model. © 2004 Wiley Periodicals, Inc. Complexity 9: 24–30, 2004},
year = {2004}
}

@article{doi:10.1142/S0129183104006728,
author = {Fortunato, Santo},
title = {UNIVERSALITY OF THE THRESHOLD FOR COMPLETE CONSENSUS FOR THE OPINION DYNAMICS OF DEFFUANT et al.},
journal = {International Journal of Modern Physics C},
volume = {15},
number = {09},
pages = {1301-1307},
year = {2004},
doi = {10.1142/S0129183104006728},

URL = { 
        https://doi.org/10.1142/S0129183104006728
    
},
eprint = { 
        https://doi.org/10.1142/S0129183104006728
    
}
,
    abstract = { In the compromise model of Deffuant et al., opinions are real numbers between 0 and 1, and two agents are compatible if the difference of their opinions is smaller than the confidence bound parameter ∊. The opinions of a randomly chosen pair of compatible agents get closer to each other. We provide strong numerical evidence that the threshold value of ∊ above which all agents share the same opinion in the final configuration is 1/2, independently of the underlying social topology. }
}

@article{LORENZ2005217,
title = "A stabilization theorem for dynamics of continuous opinions",
journal = "Physica A: Statistical Mechanics and its Applications",
volume = "355",
number = "1",
pages = "217 - 223",
year = "2005",
note = "Market Dynamics and Quantitative Economics",
issn = "0378-4371",
doi = "https://doi.org/10.1016/j.physa.2005.02.086",
url = "http://www.sciencedirect.com/science/article/pii/S0378437105002955",
author = "Jan Lorenz",
keywords = "Continuous opinion dynamics, Non-negative matrices, Repeated averaging, Positive diagonal",
abstract = "A stabilization theorem for processes of opinion dynamics is presented. The theorem is applicable to a wide class of models of continuous opinion dynamics based on averaging (like the models of Hegselmann–Krause and Weisbuch–Deffuant). The analysis detects self-confidence as a driving force of stabilization."
}

@article{BENNAIM2003190,
title = "Bifurcations and patterns in compromise processes",
journal = "Physica D: Nonlinear Phenomena",
volume = "183",
number = "3",
pages = "190 - 204",
year = "2003",
issn = "0167-2789",
doi = "https://doi.org/10.1016/S0167-2789(03)00171-4",
url = "http://www.sciencedirect.com/science/article/pii/S0167278903001714",
author = "E. Ben-Naim and P.L. Krapivsky and S. Redner",
keywords = "Bifurcations and patterns, Compromise process, Opinion dynamics model",
abstract = "We study an opinion dynamics model in which agents reach compromise via pairwise interactions. When the opinions of two agents are sufficiently close, they both acquire the average of their initial opinions; otherwise, they do not interact. Generically, the system reaches a steady state with a finite number of isolated, non-interacting opinion clusters (“parties”). As the initial opinion range increases, the number of such parties undergoes a periodic sequence of bifurcations. Both major and minor parties emerge, and these are organized in alternating pattern. This behavior is illuminated by considering discrete opinion states."
}

@article{doi:10.1142/S0129183105008126,
author = {Fortunato, Santo and Latora, Vito and Pluchino, Alessandro and Rapisarda, Andrea},
title = {VECTOR OPINION DYNAMICS IN A BOUNDED CONFIDENCE CONSENSUS MODEL},
journal = {International Journal of Modern Physics C},
volume = {16},
number = {10},
pages = {1535-1551},
year = {2005},
doi = {10.1142/S0129183105008126},

URL = { 
        https://doi.org/10.1142/S0129183105008126
    
},
eprint = { 
        https://doi.org/10.1142/S0129183105008126
    
}
,
    abstract = { We study the continuum opinion dynamics of the compromise model of Krause and Hegselmann for a community of mutually interacting agents by solving numerically a rate equation. The opinions are here represented by two-dimensional vectors with real-valued components. We study the situation starting from a uniform probability distribution for the opinion configuration and for different shapes of the confidence range. In all cases, we find that the thresholds for consensus and cluster merging either coincide with their one-dimensional counterparts, or are very close to them. The symmetry of the final opinion configuration, when more clusters survive, is determined by the shape of the opinion space. If the latter is a square, which is the case we consider, the clusters in general occupy the sites of a square lattice, although we sometimes observe interesting deviations from this general pattern, especially near the center of the opinion space. }
}

@inproceedings{10.5555/2615731.2615778,
author = {Tsang, Alan and Larson, Kate},
title = {Opinion Dynamics of Skeptical Agents},
year = {2014},
isbn = {9781450327381},
publisher = {International Foundation for Autonomous Agents and Multiagent Systems},
address = {Richland, SC},
booktitle = {Proceedings of the 2014 International Conference on Autonomous Agents and Multi-Agent Systems},
pages = {277–284},
numpages = {8},
keywords = {opinion dynamics, innovation diffusion, social simulation, social networks, cognitive convergence, agent-based models, information propagation, homophily, degree-based voter model},
location = {Paris, France},
series = {AAMAS ’14}
}

@ARTICLE{10.3389/fphy.2015.00017,
  
AUTHOR={Sobkowicz, Pawel},   
	 
TITLE={Extremism without extremists: Deffuant model with emotions},      
	
JOURNAL={Frontiers in Physics},      
	
VOLUME={3},      

PAGES={17},     
	
YEAR={2015},      
	  
URL={https://www.frontiersin.org/article/10.3389/fphy.2015.00017},       
	
DOI={10.3389/fphy.2015.00017},      
	
ISSN={2296-424X},   
   
ABSTRACT={The frequent occurrence of extremist views in many social contexts, often growing from small minorities to almost total majority, poses a significant challenge for democratic societies. The phenomenon can be described within the sociophysical paradigm. We present a modified version of the continuous bounded confidence opinion model, including a simple description of the influence of emotions on tolerances, and eventually on the evolution of opinions. Allowing for psychologically based correlation between the extreme opinions, high emotions and low tolerance for other people's views leads to quick dominance of the extreme views within the studied model, without introducing a special class of agents, as has been done in previous works. This dominance occurs even if the initial numbers of people with extreme opinions is very small. Possible suggestions related to mitigation of the process are briefly discussed.}
}

@article{article,
author = {Kuhn, Michael and Kirse, Christoph and Briesen, Heiko},
year = {2018},
month = {09},
pages = {164},
title = {Population Balance Modeling and Opinion Dynamics—A Mutually Beneficial Liaison?},
volume = {6},
journal = {Processes},
doi = {10.3390/pr6090164}
}
